Machine Learning-Assisted UAV Operations with UTM: Requirements, Challenges, and Solutions

Unmanned aerial vehicles (UAVs) are emerging in commercial spaces and will support many applications and services, such as smart agriculture, dynamic network deployment, and network coverage extension, surveillance and security. The unmanned aircraft system (UAS) traffic management (UTM) provides a framework for safe UAV operation integrating UAV controllers and central data bases via a communications network. This paper discusses the challenges and opportunities for machine learning (ML) for effectively providing critical UTM services. We introduce the four pillars of UTM---operation planning, situational awareness, status and advisors and security---and discuss the main services, specific opportunities for ML and the ongoing research. We conclude that the multi-faceted operating environment and operational parameters will benefit from collected data and data-driven algorithms, as well as online learning to face new UAV operation situations.

==> include/bios.tex <==
\small
\noindent
\textbf{Aly Sabri Abdalla} (asa298@msstate.edu)
is a PhD candidate in the Department of Electrical and Computer Engineering at Mississippi State University. His research interests are on scheduling and congestion control for vehicular ad-hoc and UAV networks.

\vspace{0.2cm}
\noindent
\textbf{Bodong Shang} (bdshang@vt.edu) is currently pursuing Ph.D. degree in the Bradley Department of Electrical and Computer Engineering in Virginia Tech, Blacksburg, USA. His research interests include UAV, Internet of Things, and vehicle-to-everything.

\vspace{0.2cm}
\noindent
\textbf{Vuk Marojevic} (vuk.marojevic@msstate.edu) is an associate professor in electrical and computer engineering at Mississippi State University, Starkville. His research interests include resource management, vehicle-to-everything communications and wireless security %, spectrum sharing, software radios, and wireless network virtualization 
with application to cellular communications, mission-critical networks, and unmanned aircraft systems.

\vspace{0.2cm}
\noindent
\textbf{Lingjia Liu} (ljliu@vt.edu) received his Ph.D. degree in Electrical and Computer Engineering from Texas A\&M University, USA. He is an Associate Professor in the Bradley Department of Electrical and Computer Engineering at Virginia Tech, USA. His research interests include machine learning for wireless communications, 5G and beyond, internet of things.


==> include/cases.tex <==
In this section, we will provide some of the case studies that have been conducted to test applying machine learning algorithm for enabling automated UTM functions. 

\subsection{NASA Case studies}

==> include/research.tex <==
%C-V2X Mode 4 is an ad-hoc communication mode using the PC5 air interface between UEs. In this mode, the peers are not known a priory and change dynamically because of the different trajectories of vehicles. Since infrastructure is not involved in this mode, standard LTE security mechanisms cannot be applied. 3GPP does not address the establishment of adhoc security associations in R14.
Cellular infrastructure-based and ad-hoc networking have different requirements and constraints, but security needs to be implicit to both. 
5G will enable both types of communications and 3D mobility through UAVs. It is essential to analyze and identify the key vulnerabilities and effective security mechanisms when introducing a new communications mode. %, and propose and demonstrate mechanisms to harden it. 
Research in the following areas can be leveraged to increase the security of 5G for servicing UAVs and ensuring their reliable operation:

\begin{itemize}
    \item \textbf{Physical layer techniques.} Use and leverage the diversity of the channel as well as interference mitigation techniques. Embed signatures or other unique identifiers in messages to identify legitimate UEs and legitimate messages. %5G will need to leverage PHY layer security, which can relieve implementing computing intensive encryption and other security mechanisms where not practical.
    
    \item \textbf{Cross-layer techniques.} Modify scheduling, congestion control and other 5G procedures to improve their robustness and increase the awareness of potential threats (e.g., scheduling messages for the purpose of enhancing distributed security awareness).
    
    \item \textbf{Edge and Cloud computing.} Use the Cloud to assist in determining fake transmitters and leverage edge computing to reduce latency and network congestion. Security mechanisms need to be implicitly in place since 5G VNFs will be sharing physical platforms where they run with other applications.
    
    %\item \textbf{Network-aided procedures.} Have the network periodically notify UEs of legitimate UEs in the area using C-V2X or parallel communications protocols, such as regular LTE.
    
    %\item \textbf{Radio environment map (REM).} Have UEs built their REMs, where processed RF spectrum activity and the information exchanged among UEs is stored and contrasted to identify anomalies.
    
    \item \textbf{Spectrum sharing security.} The aerial UEs and network nodes can regularly sense RF environments, process, and forward it for centralized or distributed RF anomaly detection. It is critical that the spectrum access system database %for shared spectrum access 
    is secure and monitored.
    
    \item \textbf{Data collection and analyses.} Data gathered from experiments or during operation needs to be processed and made available for inferring 5G operational contexts and classifying known and unknown anomalies. %can ML can be effectively employed to analyze huge amounts of data and classify it. When either the normal behavior is known or the attacks, ML tools can be trained to distinguish between normal and abnormal activity.
    
    \item \textbf{Sensor fusion.} Physical attributes, past messages, environmental contexts, etc. and information coming from multiple sensors can be used to validate messages, weigh decisions and dynamically update node and information thrust metrics. %Message content for consistency 
\end{itemize}

%Research has shown that combining multiple sources of data can help identifying and overcoming a threat. %An example of this is jointly processing several of the widely used performance measurement counters and key performance indicators in cellular networks to identify a specific source of interference. 

% The following tools can be leveraged for accelerating research, testing, and standardization:

% \begin{itemize}
%     \item Software-defined radios and open-source software,
%     \item Laboratory and field experiments, providing data for researchers to use, 
%     \item Crowdsourcing, allowing distributed development and testing as well as contributions to specifications,
%     \item Specifications with more dynamic contributions,
%     \item Regular firmware and software updates and secure software downloads and installations for radios and wireless networking equipment and at a rate comparable to IT systems, 
%     \item Use of virtualization technology to enable dynamic network reconfiguration and security as a service. 

% \end{itemize}




One of the main challenges is the real-time nature of the data and the limited resources (time, RF bandwidth, and processing power) that are available. Moreover, the interference or attack may change. Therefore, one solution will not fit all cases and a single approach may result ineffective. Instead, several techniques should be combined and used in concert. For example, the UAS can do some local processing and combine it with data processed at the network edge or Cloud, or the data provided by the network. 


==> include/table.tex <==

\begin{table*}[ht]
\centering
\caption{ML opportunities and techniques for the UTM functions of Fig. 1}
\label{tab:my-table}
%\resizebox{0.5\textwidth}{!}%{%
%\begin{tabular}{|c|c|c|}
{\begin{tabular}{|p{2cm}|p{6.6cm}|p{7.8cm}|}
\hline

\textbf{Function} & \textbf{ML opportunities} & \textbf{ML techniques}            
\\ \hline


\vspace{-0.02 in}
Operation Planning  &
\vspace{-0.05 in}

%& \begin{tabular}[c]{@{}c@{}}
\vspace{-0.05 in}
\begin{list}{\labelitemi}{\leftmargin=0.2em}
    \item {\small Dynamic trajectory planning in new situations}%\\ \\
    \item {\small Lack of prior information of paths, needed to classify}
    %\\ \\ 
    \item {\small Adjustment of paths as a function of UAV states}%\\ \\
    \item {\small Flight optimization on the fly}%\end{tabular}
    \vspace{-0.1 in}
\end{list}    

    &
    %\begin{tabular}[c]{@{}c@{}}
    %
    \vspace{-0.09 in}
\begin{list}{\labelitemi}{\leftmargin=0.2em}
    \item {\small RL when no a priori data is available or the environment changes~\cite{RLPATHprediction}.}%\\ \\
    \item {\small DRL to processes many  parameters~\cite{PathOptimize}.}%\end{tabular}         
   
    \vspace{-0.1 in}
    \end{list}  
    
    \\ \hline
    
    \vspace{0.001 in}
Situational Awareness  & %\begin{tabular}[c]{@{}c@{}}
\vspace{-0.05 in}

\vspace{-0.05 in}
\begin{list}{\labelitemi}{\leftmargin=0.2em}
\item {\small Weather condition awareness and prediction}%\\ \\ 
\item {\small Terrain awareness and assessment of communications and safety implications}%\\ \\ 
\item {\small Obstacle awareness}%\end{tabular} 
    \vspace{-0.1 in}
\end{list}

&
%\begin{tabular}[c]{@{}c@{}}
\vspace{-0.09 in}
\begin{list}{\labelitemi}{\leftmargin=0.2em}
\item {\small CNN to estimate the 3D wind flow for trajectory adjustment~\cite{WindCNN}.}%\\ \\ 
\item {\small SVM to classify LoS and NLoS link conditions of the UAV along the flight~\cite{TerrianSVM}.}%\\ \\
\item {\small DL, RL, and CNN for obstacle detection and avoidance~\cite{ObstacleDRL}.}%\end{tabular}          
    \vspace{-0.1 in}
\end{list}

\\ \hline


%\begin{tabular}[c]{@{}c@{}}
 \vspace{0.001 in}
Failure Detection and Recovery  &
%\end{tabular} 
\vspace{-0.05 in}

%\begin{tabular}[c]{@{}c@{}}
\vspace{-0.05 in}
\begin{list}{\labelitemi}{\leftmargin=0.2em}
\item {\small Failure detection (UAV, comm. network, ground users)}%\\ \\ 
%\vspace{0.1 in}
\item {\small Failure assessment and impacts classifications}%\\ \\
\vspace{0.15 in}
\item {\small Failure recovery}%\end{tabular} 
    \vspace{-0.1 in}
\end{list}

&
%\begin{tabular}[c]{@{}c@{}}
\vspace{-0.09 in}
\begin{list}{\labelitemi}{\leftmargin=0.2em}
\item {\small Supervised learning that uses historical datasets for prediction of future failures~\cite{HWFailure,HWFailure2}.}%\\ \\
\item {\small Artificial neural networks (ANNs) are the most common model for risk assessment in the UAS network~\cite{MLRISK}.}%\\ \\ 
\item {\small RL can be used to define the optimum fault-tolerant recovery policy against different failures or attacks~\cite{FailurReco}.}%\end{tabular} \\
    \vspace{-0.1 in}
\end{list}

\\ \hline


 \vspace{0.001 in}
Remote Identification   &
\vspace{-0.05 in}

\vspace{-0.05 in}

\begin{list}{\labelitemi}{\leftmargin=0.2em}
\item {\small Data security and analysis}                      \vspace{-0.1 in}
\end{list}
                
& 

%\begin{tabular}[c]{@{}c@{}}

\begin{list}{\labelitemi}{\leftmargin=0.2em}
\vspace{-0.09 in}
\item {\small Data mining techniques to provide a secure analytic of dynamic streams of data~\cite{datamining}.}%\end{tabular}                    
\vspace{-0.1 in}
\end{list}

\\ \hline
\end{tabular}%
}
\end{table*}
